Uncertainty Quantification in CNN-Based Surface Prediction Using Shape Priors

Surface reconstruction is a vital tool in a wide range of areas of medical image analysis and clinical research. Despite the fact that many methods have proposed solutions to the reconstruction problem, most, due to their deterministic nature, do not directly address the issue of quantifying uncertainty associated with their predictions. We remedy this by proposing a novel probabilistic deep learning approach capable of simultaneous surface reconstruction and associated uncertainty prediction. The method incorporates prior shape information in the form of a principal component analysis (PCA) model. Experiments using the UK Biobank data show that our probabilistic approach outperforms an analogous deterministic PCA-based method in the task of 2D organ delineation and quantifies uncertainty by formulating distributions over predicted surface vertex positions.

==> timsdefs.tex <==
%%% Tim's Stuff %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\x{{\vect{x}}}
\def\y{{\vect{y}}}
\def\z{{\vect{z}}}
\def\c{{\vect{c}}}
\def\s{{\vect{s}}}
\def\p{{\vect{p}}}
\def\q{{\vect{q}}}
\def\r{{\vect{r}}}
\def\u{{\vect{u}}}
\def\v{{\vect{v}}}
\def\w{{\vect{w}}}
\def\n{{\vect{n}}}
\def\m{{\vect{m}}}
\def\O{{\vect{o}}}

\def\scrpax{{\vect{p}^*\!}}

\def\e{{\mbox{e}}}

\newcommand{\B}[1]{\mathbf{#1}}   % switch to bold math font

\def\bAlpha{\B{\alpha}}
\def\bBeta{\B{\beta}}

\def\zeroset{{0\!\!\!/}}

%\newcommand{\IR}{\mbox{$\mathds{R}$}}
\newcommand{\IR}{\mbox{I$\!$R}}
\newcommand{\IN}{\mbox{$\mathds{N}$}}
\newcommand{\IZ}{\mbox{$\mathds{Z}$}}
\newcommand{\IC}{\mbox{$\mathds{C}$}}

% for EG style:
\newlength{\maxfigwidth}
\setlength{\maxfigwidth}{\columnwidth}

% \setlength{\parskip}{0pt}  % usually a good idea, but not for EG style :-(

% Three possible type settings for transposed matrices:
%
\def\tsuper{^{\top\!}}
%\def\tsuper{^{T\!}}
%\def\tsuper{^{\rm T\!}}

% Tiny transpose version for large matrices:
\def\ttsuper{^{\!\mbox{\tiny$\top$}\!}}

% Choose, what matrix type you like (brackets or
% parantheses)
%
%\def\bmatrix#1{\left[\matrix{#1}\right]}
\def\bmatrix#1{\pmatrix{#1}}

\def\tm{\mbox{$^{\!\mbox{\tiny TM}}$}}


% The adobe fonts lead to some spacing errors. So, I defined the
% following corrected expressions:
\def\pj{{\p\!_j}}         % instead of \p_j


\newcommand*{\nopicture}[2][0.9\linewidth]{%
  \framebox{\parbox[b][0.6\linewidth][c]{#1}{
      \begin{center}#2\end{center}
      }}
  }

\newcommand*{\nopicturehalf}[2][0.42\linewidth]{%
  \framebox{\parbox[b][0.4\linewidth][c]{#1}{
      \begin{center}#2\end{center}
      }}
  }

\newcommand*{\nopicturethird}[2][0.3\linewidth]{%
  \framebox{\parbox[b][0.33\linewidth][c]{#1}{
      \begin{center}#2\end{center}
      }}
  }

\newcommand*{\nopicturedoubleheight}[2][0.9\linewidth]{%
  \framebox{\parbox[b][1.2\linewidth][c]{#1}{
      \begin{center}#2\end{center}
      }}
  }

\newcommand*{\nopicturehalfdoubleheight}[2][0.45\linewidth]{%
  \framebox{\parbox[b][0.8\linewidth][c]{#1}{
      \begin{center}#2\end{center}
      }}
  }

\newcommand*{\nopicturethirddoubleheight}[2][0.3\linewidth]{%
  \framebox{\parbox[b][0.67\linewidth][c]{#1}{
      \begin{center}#2\end{center}
      }}
  }

% remarks:
%\def\rem#1{{[\textbf{\textit{#1}}]}}
\def\rem#1{}
% section wording tasks:
%\def\scttask#1{\break{\small\textit{[#1]}}}
\def\scttask#1{}

%\def\new{\bf}
\def\new{}

\def\myindent{\noindent\rule{0pt}{1pt}\hskip\parindent}

%
%   % enumerate-Stil
%
%   %% Kursiv-romans
%   %\def\theenumi{({\it\roman{enumi}}\/)}
%
%   % aufrechte Kursiv-romans (muesste {u} statt {it} sein) -- krieg
%   % ich nicht hin
%   %\def\theenumi{({\usefont{OT1}{cmr}{m}{it}\roman{enumi}}\/)}
%
%   \def\theenumi{({\roman{enumi}})}
%
%   \def\labelenumi{\theenumi}
%

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


